Dual Mechanism Priming Effects in Hindi Word Order

Word order choices during sentence production can be primed by preceding sentences. In this work, we test the DUAL MECHANISM hypothesis that priming is driven by multiple different sources. Using a Hindi corpus of text productions, we model lexical priming with an n-gram cache model and we capture more abstract syntactic priming with an adaptive neural language model. We permute the preverbal constituents of corpus sentences, and then use a logistic regression model to predict which sentences actually occurred in the corpus against artificially generated meaning-equivalent variants. Our results indicate that lexical priming and lexically-independent syntactic priming affect complementary sets of verb classes. By showing that different priming influences are separable from one another, our results support the hypothesis that multiple different cognitive mechanisms underlie priming.

==> background.tex <==
\section{Background}\label{sect:backg}

% \rmred{This section presents a brief background on the theory of surprisal and dependency length minimization proposed in the comprehension literature. We also provide a summary of the various cognitive features used in this work to study preverbal constituent ordering.}

\subsection{Surprisal Theory}

Surprisal Theory \citep{hale2001,levy2008} posits that comprehenders construct probabilistic interpretations of sentences based on previously encountered structures. Mathematically, the \textit{surprisal} of the ${k}^{th}$ word, $w_k$, is defined as the negative log probability of $w_k$ given the preceding context: %, as computed over either word sequences or syntactic configurations:% which can either consist of a \textit{sequence of words} or a \textit{syntactic tree} as shown below:%(see Equation \ref{eq1}).%It quantifies the comprehension difficulty of an observation as the amount of information that observation introduces. %offers a surprisal metric (an entity of mental surprise) to account for the comprehension difficulty of a sentence.

\begin{small}
\begin{equation}{\label{eq1}}
S_{k}= -\log P(w_{k}|w_{1...k-1}) = \log \frac{P(w_{1}...w_{k-1})}{P(w_{1}...w_{k})}
\end{equation}
\end{small}

\begin{comment}
\begin{small}
\begin{equation}{\label{eq2}}
S_{k+1}= -\log P(w_{k+1}|T) = \log \frac{\sum_{T}^{} P(T, w_{1}...w_{k})}{\sum_{T}^{} P(T, w_{1}...w_{k+1})}
\end{equation}
\end{small}
\end{comment}

These probabilities can be computed either over word sequences or syntactic configurations and reflect the information load (or predictability) of $w_k$. Both versions of surprisal predict eye-movements in reading times~\citep{levy2008,DembergKeller2008,staub2015} as well as spontaneous speech word durations~\citep{demberg-sayeed-2012,dammalapati2021expectation}.

\subsection{Dependency Locality Theory}

Dependency locality theory \citep{gibson00} has been shown to be effective at predicting the comprehension difficulty of a sequence, with shorter dependencies generally being easier to process than longer ones \citep[][cf.\ \protect\citeauthor{DembergKeller2008}, \citeyear{DembergKeller2008}]{Temperley2007,futrell2015,Liu2017}. In this work, we defined dependency length as the number of intervening words between head and dependent units in a dependency tree~\citep{Temperley08,cog:raja}. 
% It offers two processing measures, viz., storage cost and integration cost, to model syntactic complexity. Storage cost (forward-looking cost) deals with the cost incurred in maintaining the incomplete syntactic dependencies in memory. In contrast, integration cost (backward-looking cost) captures the cost of connecting a word in the memory to an upcoming word with which it has its syntactic linkages. 
%Dependency length and reading times (metric for processing difficulty) have been shown to be correlated in sentence comprehension literature~\citep{warrengibson02,husain2015}. 
% For Hindi, \citet{vasishth2003working} showed that non-canonical word order (OSV) viz., indirect object (IO) fronted and direct object (DO) fronted constructions have higher reading times at innermost verb than their corresponding canonical forms. He further elucidates that fronting of indirect and direct object leads to processing of more number of new discourse referents between the head and the dependents as compared to canonical counterpart; thus incurring higher consumption of memory resources resulting in larger comprehension difficulty. Further experiments using eye-tracking reading data suggest weak effects of locality \citep{husain2015,agrawal2017expectation}. Moreover, with SPR data,~\citet{husain2014expectations} show an interaction with expectation effects such that strong expectation cancels locality considerations in Hindi. 
% In this work, we use dependency length measure as a control variable to account for syntactic complexity in constituent ordering. 

\subsection{Information Status}

Information structure strongly influences syntactic choice~\citep{halliday1970language}. Languages generally prefer to mention \textit{given} referents, from earlier in the discourse, before introducing \textit{new} ones~\citep{Clark-Haviland77,chafe1976givenness,kaiser2004role}. The explanation for this is that given information is more accessible compared to new information, so providing the given information first provides a more robust context to ease processing of the new referents~\citep{Arnold00heaviness,bockIrwin1980}. 
% Therefore, \textit{Give-New} ordering could be a result of accessibility effects~\citep{Arnold00heaviness,bockIrwin1980}. In this regard, \cite{slevc2011} further expounded using production experiments that the accessibility effect diminishes under a working memory load condition and is susceptible to interference with other information in the memory. In a recent study on factors affecting the acceptability of object fronting in German~\citep{wierzba2020factors}, the authors found a robust effect of object fronting under discourse-given and definite pronoun conditions using multiple acceptability rating experiments. 
%The first sentence (\ref{ex:h1b}) is corpus reference sentence and other one (\ref{ex:h2b}) is the alternative variant expressing same idea.

\begin{comment}
\begin{small}
\begin{exe}

  \ex \label{ex:prev-sent}
  {\label{ex:h1a}
    \gll {\underline{amar ujala}-ki} {bhumika} {nispaksh} {rehti} {hai} \textbf{(Previous sentence)}\\
         {Amar Ujala-\textsc{gen}} {role} {unbiased} {remain} {be\textsc{.prs.sg}}\\
     \glt Amar Ujala's role remains unbiased.}

\end{exe}
\end{small}

\begin{small}
\begin{exe}

  \ex \label{ex:hindi-introb}
  \begin{xlist}
  \ex[]{\label{ex:h1b}
    \gll {\underline{amar ujala}-ko} {\bf yah} {sukravar-ko} {daak-se} {prapt} {hua} [Given-Given = 0] \textbf{(Reference)}\\
         {Amar Ujala-\textsc{acc}} {it} {friday-on} {post-\textsc{inst}} {receive} {be\textsc{.pst.sg}}\\
     \glt Amar Ujala received it by post on Friday.}
  \ex[] {\label{ex:h2b} {{\bf yah} \underline{{amar ujala}}-ko sukravar-ko daak-se prapt hua} [Given-Given = 0] \textbf{(Variant)}}
  %\ex[] {\label{ex:h3b} {sukravar-ko {\bf yah} \underline{amar ujala}-ko daak-se prapt hua} [New-Given = -1] \textbf{(Variant)}}
  \end{xlist}

\end{exe}
\end{small}
\end{comment}














